A k-mer Based Approach for SARS-CoV-2 Variant Identification

With the rapid spread of the novel coronavirus (COVID-19) across the globe and its continuous mutation, it is of pivotal importance to design a system to identify different known (and unknown) variants of SARS-CoV-2. Identifying particular variants helps to understand and model their spread patterns, design effective mitigation strategies, and prevent future outbreaks. It also plays a crucial role in studying the efficacy of known vaccines against each variant and modeling the likelihood of breakthrough infections. It is well known that the spike protein contains most of the information/variation pertaining to coronavirus variants. In this paper, we use spike sequences to classify different variants of the coronavirus in humans. We show that preserving the order of the amino acids helps the underlying classifiers to achieve better performance. We also show that we can train our model to outperform the baseline algorithms using only a small number of training samples ($1\%$ of the data). Finally, we show the importance of the different amino acids which play a key role in identifying variants and how they coincide with those reported by the USA's Centers for Disease Control and Prevention (CDC).

==> Intro_Related_Approach_Points.tex <==
Classifying chemicals based on their carcinogenicity~\cite{helma2001predictive}, determining which kind of community is represented by a friendship network~\cite{yanardag2015deep}, and detecting discontinuities within instant messaging interactions~\cite{berlingerio2013network} are just a few examples of problems that can be tackled via graph comparison. The solutions to these problems are contingent on the computation of a similarity (or distance) measure between a pair of graphs. Unfortunately, evidence suggests that constructing such a measure efficiently is a difficult task. For instance, even the best-known solution for determining whether two graphs are isomorphic takes quasi-polynomial time, and computing Graph Edit Distance, the minimum number of node/edge addition/deletions to transform one graph into another, is an \textsc{NP-Hard} problem.

% In lieu of comparing a pair of graphs directly, a pragmatic approach is to construct fixed dimensional descriptors (vector embeddings) for these graphs, thereby allowing the use of classical data mining algorithms that operate on vector spaces. This technique has been explored extensively in the past, and existing models can be split into two categories: (1) supervised models, which use deep learning methods to construct vector embeddings for a dataset based on optimizing a given objective function~\cite{morris2019weisfeiler,wu2019comprehensive,xu2018powerful}, and (2) unsupervised models, which are based on graph-theoretic properties such as degree, the Laplacian eigenspectrum, or distribution of a fixed number of sub-graphs~\cite{sge,kondor2016multiscale,shervashidze2011weisfeiler,shervashidze2009efficient,tsitsulin2018netlsd,verma2017hunt}.


Evaluating pairwise similarity/distance between graphs is a fundamental building block for analysis of large graphs. In the so-called direct approach to compute pairwise proximity the entire structure of both graphs are considered. A simple and most well-known distance measure between graphs is the {\em Graph Edit Distance} (\textsc{ged}) ~\cite{sanfeliu1983distance}. \textsc{ged}, like edit distance between sequences counts the number of insertions, deletion, and substitution of vertices and/or edges that are needed in order to transform one graph to the other. Running times of computing \textsc{ged} between two graphs is computationally prohibitive, which makes it applicable to graphs of very small orders (number of vertices) and sizes (number of edges). Another distance measure based on the permutation of vertices of one graph such that an error-norm between the adjacency matrices of two graphs ~\cite{Beg2018Scalable} is minimum. Computing this distance and even relaxation of this distance is computationally expensive \cite{babai2016graph,bento2018family}. When there is a valid bijection between vertices of the two graphs, then a similar measure, \textsc{DeltaCon} proposed in ~\cite{faloutsos2013deltacon} yields excellent results. However, the requirement of a valid bijection limits the applicability of \textsc{DeltaCon} only to a collection of graphs on the same vertex set.



In the representation learning approach for graph analysis, graphs are first mapped into a fixed-dimensional vector space. Vector space machine learning algorithms are employed using a pairwise distance measure between the vector representations of graphs. We discuss three broad classes of graph representation learning. 

The kernel-based machine learning methods represent each non-vector data item to a fixed and high dimensional vector. These feature vectors are based on counts (spectra) of all possible sub-structures of some fixed magnitude in the data item. A kernel function is then defined, that usually is the dot-product of the pair of feature vectors. The pairwise kernel values between all objects, a positive semi-definite matrix, is used as a similarity measure in the machine learning algorithm (e.g. SVM and kernel PCA). Explicit construction of feature vectors is computationally very expensive due to their large dimensionality, therefore in the so-called {\em kernel trick} kernel values are directly evaluated based on objects. Kernel methods have yielded great successes for various kind of objects such as images and sequences ~\cite{Bo_ImageKernel,Kuksa_SequenceKernel,Farhan_SequenceKernel}. Computational and space complexity of evaluating and storing the kernel matrix make kernel based methods infeasible for large datasets of massive graphs.


Another approach of representation learning is to train a neural network for embedding objects into Euclidean space. The goal here is to map `similar' objects to `close-by' points in $\mathbb{R}^d$. Deep learning based methods together with domain-specific techniques have been successfully used for embedding nodes in a network \cite{duran2017learning,grover2016node2vec,cao2015grarep}, graphs \cite{xu2018powerful, morris2019weisfeiler,Yang2020jane,yang20183} and texts \cite{Shakeel2019MultiBilingual,Shakeel2020Multi,Shakeel2020LanguageIndependent}. Vector-space based machine learning methods are then employed on these embedding for data analysis in various disciplines. These approaches, however are very data hungry and are computationally prohibitive~\cite{wu2019comprehensive}, hindering their scalability to graphs of large orders and sizes.

The descriptor based representation learning paradigm differs from kernel methods as the dimensionality of the feature vectors is relatively much smaller than the kernel-based features. While, unlike neural network based models the features are hand-picked using domain specific knowledge and are thus explainable and are computed using efficient graph algorithms. Descriptors have been proposed for sequences \cite{atzori2014electromyography,ullah2020effect} and electricity consumptions \cite{ali2019short,Ali2020ShortTerm, ali2020fair}.



In many supervised and unsupervised machine learning tasks, for example, classification, clustering, anomaly detection, etc. the fundamental building block is a {\em `meaningful'} proximity measure between pairs of sequences. Generally, sequences are first mapped into fixed dimensional feature vectors based on the descriptive statistics of their contents. In one of the most successful approaches, the feature vector is the spectrum (count) of all $k$-length sub-sequences, $k$-mers, present exactly or inexactly (up to $m$ mismatches) in the sequence. For an alphabet $\Sigma$, sequences are mapped into $|\Sigma|^k$ dimensional vector space using sub-string \emph{feature map} \cite{leslie2002spectrum,leslie2002mismatch}. A \emph{kernel function} is then defined that takes as input a pair of feature vectors (images of two sequences under the feature map) and returns a real-valued similarity score between the pair \cite{hofmann2008kernel, souza2010kernel}. For two sequences $X$ and $Y$, the $(k,m)$-mismatch kernel value, $K(X,Y|k,m)$, is the dot product of the respective feature vectors containing the count of $k$-mers present up to $m$-mismatches in $X$ and $Y$.

The exponential dimensions ($|\Sigma|^k$) of the feature space make the explicit transformation of sequences computationally prohibitive. The {\em Kernel trick} is an approach that computes inner product between feature vectors without explicitly constructing the feature vectors. 

The runtime of computing $K(X,Y|k,m)$ under the trie-based framework is $O((|X| +|Y|)k^{m+1}|\Sigma|^m)$ \cite{leslie2002mismatch}. This is clearly only feasible for small $|\Sigma|$, $k$, and $m$ and can not scale for music data, where $|\Sigma| \in \{1024,2048\}$ (for text data, $|\Sigma|$ can be even larger). It has been shown that large values of the independent variables, $k$ and $m$ improve accuracy of analysis \cite{Kuksa2011PhdThesis, kuksa2009scalable}.



Sequential data is ubiquitous in machine learning, data mining, and pattern recognition and sequence analysis has numerous applications in a wide array of fields. Considering a text document as a sequence of words and then categorizing text into classes based on its topic, such as sports, science, etc., is a common task in natural language processing \cite{Shakeel2019MultiBilingual}. Sequence homology (shared ancestry) detection between a pair of protein or DNA sequences and prediction of the three-dimensional structure of proteins are important tasks in bioinformatics and biotechnology. Sequence classification algorithms have been applied to both of these problems with great success. Music data, originally a real-valued signal is discretized using the MFCC features, is another form of sequential data \cite{tzanetakis2002musical}.  Recognizing the genre of a music sequence, with no annotation, is an interesting classification problem. Similarly, in chemistry, sequences of monomers are analyzed to identify polymers morphology and design of nanomaterials \cite{Aldaye2008Assembling}.

Various methods have been proposed to compute the pairwise similarity between two sequences. In the computational biology community, pairwise local and global alignment similarity scores between sequences were used traditionally for sequence analysis, like the local and global alignment \cite{cristianini2000introduction,waterman1991computer}. In the representation learning methods, objects are mapped to Euclidean space such that `similar' objects have a small distance in the new space. The low dimensionality of the feature space allows efficient object mapping and machine learning algorithms are employed on these representations. This approach has been used  for graphs ~\cite{berlingerio2013network, sge, hassan2020estimating, verma2017hunt, tsitsulin2018netlsd}, EMG signals \cite{atzori2014electromyography,ullah2020effect}, nodes with attributes in social networks \cite{hamilton2017inductive, hou2019representation, Ali2020Predicting} and consumers' electricity usage patterns \cite{Ali2019Short}. More recent but computationally expensive methods employ deep networks together with domain-specific techniques for embedding nodes \cite{duran2017learning}, graphs \cite{xu2018powerful, morris2019weisfeiler} and texts \cite{Shakeel2019MultiBilingual,Shakeel2020Multi,Shakeel2020Language}. A deep Bayesian model that uses the Gaussian process to deal with sequence kernel functions for variable-sized inputs is proposed in \cite{laradji2019Gaussian}.

In the kernel-based methods, objects are mapped to a high dimensional vector space based on occurrences of various substructures in the objects. A kernel function, usually the inner product between two feature vectors, serves as a pairwise similarity measure. Various kernels have been proposed for images \cite{Bo_ImageKernel}, graphs \cite{kondor2016multiscale, shervashidze2011weisfeiler} and many other structures. String kernel-based sequence analysis was introduced in \cite{watkins1999dynamic,haussler1999convolution}. Extending this idea, \cite{lodhi2002text} defined the {\em gappy $n$-gram kernel} and used it in conjunction with SVM \cite{vapnik1998statistical} for text classification. The main drawback of this approach is that runtime for kernel evaluations depends quadratically on the lengths of the sequences.

The $(k)$-spectrum \cite{leslie2002spectrum} and substring \cite{Vishwanathan2002fast} kernels represent sequences as fixed length vectors containing the count of occurrences of $k$-mers in them. Wildcard kernel \cite{leslie2004fast}, cluster kernel \cite{weston2003cluster}, sparse spatial kernel \cite{kuksa2008fast}, abstraction-augmented kernel \cite{kuksa2010semi}, generalized similarity kernel \cite{kuksa2012generalized} and gapped string kernel \cite{blakely2020fastsk} are several extensions of $k$-mer based kernel framework. $(k,m)$-mismatch kernels count the inexact occurrences (upto $m$ mismatches) of $k$-mers in sequences \cite{kuksa2009scalable}. These kernels yield excellent sequence analysis accuracies, however, the runtime cost of kernel evaluation was a major challenge \cite{Kuksa2011PhdThesis}.

The $(k)$-spectrum and $(k,m)$-mismatch kernels work with ($|\Sigma|^k$) dimensional feature vectors, which make the explicit transformation of strings computationally infeasible. The so-called {\em kernel trick} evaluates kernels without explicitly constructing the feature vectors. Implicit computation of kernel values for sequences was devised using a trie-based strategy  \cite{leslie2002spectrum,leslie2002mismatch}. A $(k,m)$-mismatch tree is introduced, a rooted $|\Sigma|$-ary tree of depth $k$, where each internal node has $|\Sigma|$ children corresponding to symbols in $\Sigma$. Each leaf in the mismatch tree corresponds to a $k$-mer in $\Sigma^k$ obtained by concatenating the labels on edges from root to that leaf. For each $k$-mer of a sequence, the tree is traversed in a depth-first search manner and at every node at depth $d$, a pointer is stored to the $k$-mer if its $d$-length prefix is within $m$ mismatches from the $d$-mer corresponding to that node. At each leaf, a counter is stored that counts the number of $k$-mers in the sequence that are within $m$-mismatches to the $k$-mer represented by the leaf. After this mismatch tree is populated kernel matrix is updated from each leaf node with pairwise products of counts from each pair of sequences. The runtime for computing the $(k,m)$-mismatch kernel value $K(X,Y|k,m)$ between two sequences $X$ and $Y$, under this trie-based framework, is $O((|X| + |Y|)k^{m+1}|\Sigma|^m)$. Space efficient approximation kernels for strings are proposed in \cite{TabeiYP19} while string kernels based on random features are described in \cite{lingfei2019global}. 

Kernel-based learning (machine learning methods that rely on kernels) have been proposed for the classification and regression tasks \cite{muller2001kernellearning}. Large scale kernel learning takes a computational run time of $O(n^3)$ to find the solution, where $n$ is the number of training examples. To address this challenge, many kernel approximation techniques have been proposed. Approximation using the eigen decomposition of the kernel matrix can be computed by the Nystr\"{o}m method, which reduces the computational cost of the classifiers without sacrificing accuracy \cite{Williams2000Using,Drineas2005Nystrom}. The random Fourier features method, which directly approximates the kernel function, is another approach to improve kernel learning. A comparison of the Nystr\"{o}m method and the random Fourier features method is given in \cite{Yang2012Nystrom}. Mapping of input data to randomized low-dimensional feature space to improve the training of kernel machines is described in \cite{Rahimi2007Random}. The low-rank matrix decomposition approach is widely used in the application of kernel methods to large-scale learning problems \cite{Bach2005Predictive}.





==> Makefile <==
targets = main.pdf abstract.txt

all : $(targets)

%.pdf : %.tex
	latexmk -pdf $< && latexmk -c $<

abstract.txt : main.tex
	grep -A 1000 "begin{abstract}" $< \
		| tail -n +4 \
		| grep -B 1000 "end{abstract}" \
		| head -n -3 > $@

.PHONY : clean scour
clean :
	rm -f *~
	rm -f *.aux *.bbl *.log *.out

scour : clean
	rm -f $(targets)

